Multiplicative update rules for accelerating deep learning training and increasing robustness

Even nowadays, where Deep Learning (DL) has achieved state-of-the-art performance in a wide range of research domains, accelerating training and building robust DL models remains a challenging task. To this end, generations of researchers have pursued to develop robust methods for training DL architectures that can be less sensitive to weight distributions, model architectures and loss landscapes. However, such methods are limited to adaptive learning rate optimizers, initialization schemes, and clipping gradients without investigating the fundamental rule of parameters update. Although multiplicative updates have contributed significantly to the early development of machine learning and hold strong theoretical claims, to best of our knowledge, this is the first work that investigate them in context of DL training acceleration and robustness. In this work, we propose an optimization framework that fits to a wide range of optimization algorithms and enables one to apply alternative update rules. To this end, we propose a novel multiplicative update rule and we extend their capabilities by combining it with a traditional additive update term, under a novel hybrid update method. We claim that the proposed framework accelerates training, while leading to more robust models in contrast to traditionally used additive update rule and we experimentally demonstrate their effectiveness in a wide range of task and optimization methods. Such tasks ranging from convex and non-convex optimization to difficult image classification benchmarks applying a wide range of traditionally used optimization methods and Deep Neural Network (DNN) architectures.

==> sections/biography.tex <==
\begin{IEEEbiographynophoto}{Manos Kirtas}
 obtained his B.Sc. degree in Informatics and M.Sc. degree in Artificial Intelligence from Aristotle University of Thessaloniki in 2018 and 2020, respectively. Currently he is Ph.D. candidate in domain of Deep Learning. Since February 2020 he is member of Computational Intelligence and Deep Learning research group. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Nikolaos Passalis}
received the B.Sc. degree in informatics, the M.Sc. degree in information systems, and the Ph.D. degree in informatics from the Aristotle University of Thessaloniki, Thessaloniki, Greece, in 2013, 2015, and 2018, respectively. Since 2019, he has been a post-doctoral researcher with the Computational Intelligence and Deep Learning group, AIIA lab., Dept. of Informatics, Aristotle University of Thessaloniki.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Anastasios Tefas}
received the B.Sc. in informatics in 1997 and the Ph.D. degree in informatics in 2002, both from the Aristotle University of Thessaloniki, Greece. Since 2017 he has been an Associate Professor at the Department of Informatics, Aristotle University of Thessaloniki.
From 2008 to 2017, he was a Lecturer, Assistant Professor at the same University. %From 2006 to 2008, he was an Assistant Professor at the Department of Information Management, Technological Institute of Kavala. %From 2003 to 2004, he was a temporary lecturer in the Department of Informatics, University of Thessaloniki. %From 1997 to 2002, he was a researcher and teaching assistant in the Department of Informatics, University of Thessaloniki. 
Dr. Tefas participated in 12 research projects financed by national and European funds. He has co-authored 126 journal papers, 240 papers in international conferences and contributed 8 chapters to edited books in his area of expertise. Over 7000 citations have been recorded to his publications and his H-index is 42 according to Google scholar. His current research interests include computational intelligence, deep learning, pattern recognition, statistical machine learning, digital signal and image analysis and retrieval and computer vision
\end{IEEEbiographynophoto}
